Real-Time Anomaly Detection in Video Streams

This thesis is part of a CIFRE agreement between the company Othello and the LIASD laboratory. The objective is to develop an artificial intelligence system that can detect real-time dangers in a video stream. To achieve this, a novel approach combining temporal and spatial analysis has been proposed. Several avenues have been explored to improve anomaly detection by integrating object detection, human pose detection, and motion analysis. For result interpretability, techniques commonly used for image analysis, such as activation and saliency maps, have been extended to videos, and an original method has been proposed. The proposed architecture performs binary or multiclass classification depending on whether an alert or the cause needs to be identified. Numerous neural networkmodels have been tested, and three of them have been selected. You Only Looks Once (YOLO) has been used for spatial analysis, a Convolutional Recurrent Neuronal Network (CRNN) composed of VGG19 and a Gated Recurrent Unit (GRU) for temporal analysis, and a multi-layer perceptron for classification. These models handle different types of data and can be combined in parallel or in series. Although the parallel mode is faster, the serial mode is generally more reliable. For training these models, supervised learning was chosen, and two proprietary datasets were created. The first dataset focuses on objects that may play a potential role in anomalies, while the second consists of videos containing anomalies or non-anomalies. This approach allows for the processing of both continuous video streams and finite videos, providing greater flexibility in detection.

==> Preambule.tex <==
% L'ordre compte

% Global layout
% Têtes de chapitre sans numéro de page
\makeatletter
\renewcommand\chapter{\if@openright\cleardoublepage\else\clearpage\fi
  \thispagestyle{empty}%
  \global\@topnum\z@ 
  \@afterindentfalse
  \secdef\@chapter\@schapter}
% Paragraphes en retrait (digressions)
\newenvironment{digression}[0]{
  \list{}{\listparindent 1.5em%
                      \small
                      \itemindent    \listparindent%
                      \rightmargin   \leftmargin%
                      \labelsep 0.2em%
                      \parsep        \z@ \@plus\p@}%
              \item\relax%
  }{
  \endlist%
}
\makeatother

\raggedbottom% for not too separated items
\usepackage{placeins}% for blocking figures

% Layout

\usepackage{fancyhdr}
\setlength{\headheight}{30pt}% for fancyhdr
\setlength{\parskip}{0.2\baselineskip}% 
\pagestyle{fancy}
\usepackage{scrextend}% for footnotes
\deffootnote{0em}{1.6em}{\thefootnotemark.\enskip}

\usepackage{float}
\counterwithin{figure}{section}
\renewcommand{\thefigure}{\arabic{section}.\arabic{figure}}

\usepackage{caption}
\usepackage{subcaption}

% Section pas en majuscules dans le header
\renewcommand{\sectionmark}[1]{\markright{\thesection\ #1}{}}

% Sections et figures sans numéro de chapitre
\renewcommand{\thesection}{\arabic{section}}
\renewcommand{\thesubsubsection}{\thesubsection .\arabic{subsubsection}}

% Paragraphes avec uniquement des lettres
\renewcommand{\theparagraph}{\Alph{paragraph})}

\usepackage{titling}% for author in footer
\usepackage{emptypage}% for blank pages when clearing
\usepackage{eso-pic}% pour la page de garde
\usepackage{layout}% for visualizing the layout
\usepackage{lscape}% pour avoir des pages en paysage
\usepackage{pdflscape}% pour les afficher en paysage dans les lecteurs de pdf
\usepackage[export]{adjustbox}
\usepackage{chngpage}% pour adjustwidth
\usepackage{rotating}% pour écrire verticalement (turn ou sideways)

% Tables, figures and the like

\usepackage{multirow}% row fusion
\usepackage{multicol}% for text columns
\usepackage{array}% for accessing columns
\usepackage{float}
\newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}} % centered text
\renewcommand*{\arraystretch}{1.1}% add vertical space in tables
\usepackage{tabularx, booktabs}
\usepackage{colortbl}% for cellcolor
\usepackage{longtable}% for table on many pages
\usepackage{hhline}% for double horizontal lines
\usepackage{diagbox}% for cutting a cell
\usepackage[shortlabels]{enumitem}
\providecommand{\tightlist}{%
  \setlength{\itemsep}{0pt}\setlength{\parskip}{0pt}}
\usepackage{placeins}% for blocking figures
\usepackage{graphicx}% appelé par

% Pour des tables dont certaines lignes sont de style différent avec tabular
\newcolumntype{$}{>{\global\let\currentrowstyle\relax}}
\newcolumntype{^}{>{\currentrowstyle}}
\newcommand{\rowstyle}[1]{\gdef\currentrowstyle{#1}%
  #1\ignorespaces
}

\newcolumntype{Y}{>{\currentrowstyle\centering\arraybackslash}X}

% Special parts
\usepackage[ruled, 	linesnumbered,	noend]{algorithm2e} 
\usepackage{xurl}

\usepackage[toc,page]{appendix}
\usepackage{listings}

% Suppression de fontspec et polyglossia pour pdflatex
\usepackage[english]{babel} % Remplace polyglossia

\usepackage{mathtools, amssymb, amsthm}
\DeclareMathOperator*{\argmax}{argmax} 
\DeclareMathOperator*{\argmin}{arg\,min}
\usepackage{xfrac}
\usepackage[unicode, colorlinks=true]{hyperref}

\usepackage{tocbibind} % faire apparaître la biblio dans la table des matières
\emergencystretch=1em % faire en sorte que la binlio ne deborde pas

% AFTER hyperref
\usepackage{bookmark}% fin de partie avant chapitres finaux

% Remplacer polyglossia et autres dépendances XeTeX
\usepackage[a4paper]{geometry}
\usepackage[most]{tcolorbox}

% AFTER CAPTION AND HYPERREF
\usepackage[english]{minitoc}
\setcounter{parttocdepth}{1}
\setcounter{minitocdepth}{2}
\setcounter{secnumdepth}{4}
\setcounter{tocdepth}{3}

% Sommaire de partie
\usepackage{shorttoc}

\usepackage{perpage}% pour avoir les notes renumérotées à chaque page
\MakePerPage{footnote}

\usepackage{setspace}% line spacing
\usepackage[french=guillemets]{csquotes}
\usepackage{lmodern} % Police Latin Modern, compatible avec pdflatex

% Remplacer l'utilisation de fontspec pour pdflatex
\renewcommand{\rmdefault}{lmroman} % Utilisation de Latin Modern
\renewcommand{\sfdefault}{lmss}
\renewcommand{\ttdefault}{lmtt}

\usepackage[backend=biber, natbib, maxbibnames=20, citestyle=authoryear, hyperref=true, backref=true, giveninits=true]{biblatex}
\addbibresource{these.bib} 


==> PreambuleGarde.tex <==
\makeatletter
\def\@ecole{university}
\newcommand{\ecole}[1]{\def\@ecole{#1}}

\def\@specialite{Specialty}
\newcommand{\specialite}[1]{
  \def\@specialite{#1}
}

\def\@directeur{director}
\newcommand{\directeur}[1]{
  \def\@directeur{#1}
}

\def\@encadrant{co-director}
\newcommand{\encadrant}[1]{
  \def\@encadrant{#1}
}
\def\@jurya{}{}{}
\newcommand{\jurya}[5]{
  \def\@jurya{\small #1, & \small #2 & \small #3 & \small #4 & \small #5\\}
}
\def\@juryb{}{}{}
\newcommand{\juryb}[5]{
  \def\@juryb{\small #1, & \small #2 & \small #3 & \small #4 & \small #5\\}
}
\def\@juryc{}{}{}
\newcommand{\juryc}[5]{
  \def\@juryc{\small #1, & \small #2 & \small #3 & \small #4 & \small #5\\}
}
\def\@juryd{}{}{}
\newcommand{\juryd}[5]{
  \def\@juryd{\small #1, & \small #2 & \small #3 & \small #4 & \small #5\\}
}
\def\@jurye{}{}{}
\newcommand{\jurye}[5]{
  \def\@jurye{\small #1, & \small #2 & \small #3 & \small #4 & \small #5\\}
}
\def\@juryf{}{}{}
\newcommand{\juryf}[5]{
  \def\@juryf{\small #1, & \small #2 & \small #3 & \small #4 & \small #5\\}
}
\def\@juryg{}{}{}
\newcommand{\juryg}[5]{
  \def\@juryg{\small #1, & \small #2 & \small #3 & \small #4 & \small #5\\}
}
\def\@juryh{}{}{}
\newcommand{\juryh}[5]{
  \def\@juryh{\small #1, & \small #2 & \small #3 & \small #4 & \small #5\\}
}


\def\@fulltitle{}
\newcommand{\fulltitle}[1]{
  \def\@fulltitle{#1}
}

\makeatother

\newcommand\BackgroundPic{%
	\put(0,0){%
		\parbox[b][\paperheight]{\paperwidth}{%
			\includegraphics[height=0.32\paperheight]{pagedegarde/Bordure.png}%
			\vfill
		}
	}
}
\newcommand\EtiquetteThese{%
	\put(0,0){%
		\parbox[t][\paperheight]{\paperwidth}{%
			\hfill
			\colorbox{blue}{		
				\begin{minipage}[b]{3em}
					\centering\Huge\textcolor{white}{T\\H\\E\\S\\I\\S\\}
					\vspace{0.2cm}
				\end{minipage}
			}
		}
	}
}

\makeatletter
\newcommand{\pagedegarde}{
\newgeometry{top=2cm, bottom=2cm, left=1.6cm, right=1cm}
\AddToShipoutPicture*{\BackgroundPic}
\AddToShipoutPicture*{\EtiquetteThese}
  \begin{titlepage}
  \centering
      \includegraphics[width=0.4\textwidth]{pagedegarde/paris8.png}
      \hfill
      \includegraphics[width=0.2\textwidth]{pagedegarde/logo}\\
    \vspace{0.7cm}
      {\Large Doctoral School : Cognition, Langage, Interaction}\\
    \vspace{0.45cm}
    {\Huge \vspace{0.3cm}THESIS}\\
    \vspace{0.5cm}
    {\bfseries to obtain the degree of Doctor awarded by}\\
    \vspace{0.65cm}
    \huge\bfseries \@ecole\\
    \vspace{0.5cm}
    \Large{\bfseries Specialty \textit{\@specialite}}\\
    \vspace{0.8cm}
    \normalsize
    \textit{presented and publicly defended by}\\
    \vspace{0.5cm}
    {\Large {\bfseries \@author}} \\
    \vspace{0.4cm}
    	le \@date \\
    \vspace{0.8cm}
       {\LARGE \color[rgb]{0,0,1} \bfseries{\@fulltitle}} \\
    \vspace{0.8cm}
       Thesis Director : {\bfseries \@directeur}\\
    \vspace{0.5cm}
        Co-thesis Director : {\bfseries \@encadrant}\\
    \vspace{0.5cm}

\begin{tabular}{>{\bfseries}llllr}
		\large Jury\\
		\tabularnewline
		\@jurya
		\@juryb
		\@juryc
		\@juryd
		\@jurye
		\@juryf\\
		\@juryg
	\end{tabular}


	\vfill
	
	\textbf{LIASD Laboratory}\\
  \end{titlepage}




\restoregeometry  
  
  
}
\makeatother

